Deep Learning for Free-Hand Sketch: A Survey

Free-hand sketches are highly illustrative, and have been widely used by humans to depict objects or stories from ancient times to the present. The recent prevalence of touchscreen devices has made sketch creation a much easier task than ever and consequently made sketch-oriented applications increasingly popular. The progress of deep learning has immensely benefited free-hand sketch research and applications. This paper presents a comprehensive survey of the deep learning techniques oriented at free-hand sketch data, and the applications that they enable. The main contents of this survey include: (i) A discussion of the intrinsic traits and unique challenges of free-hand sketch, to highlight the essential differences between sketch data and other data modalities, e.g., natural photos. (ii) A review of the developments of free-hand sketch research in the deep learning era, by surveying existing datasets, research topics, and the state-of-the-art methods through a detailed taxonomy and experimental evaluation. (iii) Promotion of future work via a discussion of bottlenecks, open problems, and potential research directions for the community.

==> tex_files/architecture_comparison2.tex <==

\begin{table*}[!tb]
\caption{
 Recognition accuracy comparison for different network architectures, on the subset (randomly selected 414k sketches~\cite{xu2019multi}) of QuickDraw~\cite{ha2018sketchrnn}. 
}

\label{table:comparison_on_recognition}

\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{c | l | c | c | c | c | r }
\hline
 \multicolumn{2}{c|}{\multirow{2}{*}{Architecture \& Network}}  & \multirow{2}{*}{Input} & \multicolumn{3}{c|}{Recognition Accuracy} & \multirow{2}{*}{\tabincell{c}{Parameter \\ Amount}}  \\
  \cline{4-6}
\multicolumn{2}{c|}{}   & & acc.@1 & acc.@5 & acc.@10 &   \\
 \hline
 %\multirow{17}{*}{Convolutional Neural Networks (CNNs)}
\parbox[t]{2mm}{\multirow{17}{*}{\rotatebox[origin=c]{90}{CNNs}}}
& AlexNet~\cite{krizhevsky2012imagenet} & \multirow{17}{*}{picture} & {0.6808} & {0.8847} & {0.9203} & 58,417,305  \\

& VGG-11~\cite{simonyan2014very} &   & {0.6743} & {0.8814} & {0.9191} & 130,179,801 \\

& VGG-13~\cite{simonyan2014very} &   &  0.6808  & 0.8881 & 0.9232 &  130,364,313 \\

& VGG-16~\cite{simonyan2014very} &   & 0.6837 & 0.8889  & 0.9253 &  135,674,009 \\

& VGG-19~\cite{simonyan2014very} &   &  0.6908 & 0.8839  & 0.9208 &  140,983,705 \\


& Inception V3~\cite{szegedy2016rethinking} & &  {0.7422} & {0.9189} & {0.9437}  & 25,315,474  \\

& ResNet-18~\cite{he2016deep} &  & {0.7164} & {0.9072} & {0.9381}  & 11,353,497  \\

& ResNet-34~\cite{he2016deep} &   & {0.7154} & {0.9083} & {0.9375}  & 21,461,657  \\

& ResNet-50~\cite{he2016deep} &   & 0.7043 & 0.8987 & 0.9303  &  24,214,937  \\

& ResNet-101~\cite{he2016deep} &   & 0.7071  & 0.8992 & 0.9317 &  43,207,065  \\

& ResNet-152~\cite{he2016deep} &  & {0.6924} & {0.8973} & {0.9312} & 58,850,713 \\

& DenseNet-161~\cite{huang2017densely} & &  0.7008 & 0.8971 & 0.9302 & 27,234,105   \\

& DenseNet-169~\cite{huang2017densely} & &  0.7173 & 0.9050 & 0.9358 & 13,058,905  \\

& DenseNet-201~\cite{huang2017densely} & &  {0.7050} & {0.9013} & {0.9331} & 18,755,673  \\

& MobileNet V2~\cite{Sandler_2018_CVPR} & &   {0.7310} & {0.9161} & {0.9429} & 2,665,817 \\

\hline
%\multirow{2}{*}{Recurrent Neural Networks (RNNs)} 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{RNNs}}}
& LSTM & \multirow{4}{*}{stroke vector} &  0.6068 & 0.8416 & 0.8931 &  2,593,881  \\

& Bi-directional LSTM & & {0.6665} & {0.8820} & {0.9189} & 5,553,241  \\

& GRU & & 0.6224 & 0.8574 & 0.9055 & 2,000,473  \\

& Bi-directional GRU & & {0.6768} & {0.8854} & {0.9234} & 5,419,097  \\

  \hline
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{GNNs}}}
%\multirow{5}{*}{Graph Neural Networks (GNNs)} 
&  Graph Convolutional Network~(GCN)~\cite{kipf2017semi} & \multirow{5}{*}{stroke vector}  & {0.6800}  & {0.8869}  & {0.9224}  & 6,948,441    \\
& Graph Attention Network~(GAT)~\cite{velickovic2018graph} & & {0.6977} & {0.8952}  & {0.9298}   &   11,660,889    \\
& \textit{Vanilla} Transformer \cite{vaswani2017attention} &  & {0.5249} & {0.7802} & {0.8486} & 14,029,401   \\
& Multi-Graph Transformer (Base)~\cite{xu2019multi} &  & {0.7070} & {0.9030} & {0.9351} & 10,096,601  \\
& Multi-Graph Transformer (Large)~\cite{xu2019multi} &  & {0.7280} & {0.9106} & {0.9387} & 39,984,729 \\
\hline
Textual Convolutional Network (TCN) & TCN \cite{xu2020deep} & stroke vector &  0.5511  & 0.8020  &  0.8646  &  2,750,873   \\

\hline
\end{tabular}
}
\end{center}
\end{table*}
%--------------------------------------------------------------------------

==> tex_files/dataset_table.tex <==
\begin{table*}[!t]

\small
\caption{Summary of the representative sketch datasets. Public ``\checkmark'' denotes ``yes/available/provided''. Both `grouping'' and ``segmentation'' annotations refer to stroke-level. ``K'' and ``M'' mean ``thousand'' and ``million'', respectively. ``Cat.'' means ``category''. Stroke ``\checkmark'' denotes sketches provided as SVG files or coordinate arrays.}
\label{table:dataset_table}
\begin{center}
\resizebox{ \textwidth}{!}{
\begin{tabular}{ l | c | l | c | c | c | c | l | l }
\hline
 \tabincell{c}{Single-Modal \\ Datasets} & Public & Modalities \& Sample Amount & Cat. &  Stroke   & \tabincell{c}{Object/ \\ Scene} & \tabincell{c}{Instance \\ Pairing} & Annotations & Remarks\\
\hline

TU-Berlin~\cite{eitz2012humans} & \checkmark & 20K sketches & 250 & \checkmark  & o  &  -  & class &   \\

QuickDraw~\cite{ha2018sketchrnn} & \checkmark & 50M+ sketches & 345  & \checkmark  & o  & -  & class  &   \\

QuickDraw-5-step~\cite{choi2019sketchhelper} &  & 38M+ sketches & 345  &   & o  & -  & class  &   \\

Li \etal SPG~\cite{li2018universal} & \checkmark  & 20K sketches & 25 & \checkmark  & o  & - & class, grouping  &   \\

SketchSeg-150K~\cite{qi2019sketchsegnet+} &    & 150K sketches  & 20 & \checkmark  & o  & - & class, segmentation  & 57 semantic labels  \\

SketchSeg-10K~\cite{wang2019spfusionnet} & \checkmark & 10K sketches  & 10 &   & o  & - & class, segmentation  &  24 semantic labels \\

SketchFix-160~\cite{sarvadevabhatla2017object}  & \checkmark  &  3904 sketches  & 160  & \checkmark  &  o & -  & class, eye fixation  &   \\

\hline

&    &   &   &   &   &   &   &   \\
 \tabincell{c}{Multi-Modal \\ Datasets} & Public & Modalities \& Sample Amount & Cat. &  Stroke  & \tabincell{c}{Object/ \\ Scene} & \tabincell{c}{Instance \\ Pairing} & Annotations & Remarks\\

\hline
    &    &   &   &   &   &   &   &   \\
QMUL Shoe~\cite{Yu_2016_CVPR}    & \checkmark  & 419 sketches, 419 photos  &  1 &  & o  & \checkmark  & pairing,triplet,attribute  &  21 binary attributes  \\

QMUL Chair~\cite{Yu_2016_CVPR}    & \checkmark  & 297 sketches, 297 photos  &  1 &   & o  &  \checkmark &  pairing,triplet,attribute &   15 binary attributes \\

QMUL Handbag~\cite{Song_2017_ICCV}   &  \checkmark & 568 sketches, 568 photos  & 1  &   & o  & \checkmark  & pairing  &   \\

Sketchy~\cite{sangkloy2016sketchy}    & \checkmark  & 75K sketches, 12K photos  & 125  &  \checkmark & o  &   &  class &  12K objects \\

sketch\&UI~\cite{huang2019swire}    &   & 1998 sketches, 1998 photos & 23  &   &  o & \checkmark  &  class, pairing & UI  \\

QuickDrawExtended~\cite{dey2019doodle} & \checkmark & 330K sketches, 204K photos & 110   &   & o  &   &  class &   \\


TU-Berlin Extended~\cite{Zhang_2016_CVPR}   &    & 20K sketches, 191K photos  & 250  &   & o  &   &  class &   \\

sketch Flickr15K~\cite{hu2013performance} &  \checkmark  & 330 sketches, 15K photos  & 33 &  & o  &   & class  &   \\

Aerial-SI~\cite{jiang2017sketch,jiang2017retrieving}  &    &  400 sketches, 3.3K photos & 10  &   & o, s &   & class  & aerial scene   \\

HUST-SI~\cite{wang2016deep} &  \checkmark  & 20K sketches, 31K photos  & 250  & \checkmark  & o  &   & class  &   \\

SBSR~\cite{eitz2012sketch} &  \checkmark  & 1814 sketches, 1814 3D models & 161  &   & o  &   & class  &   \\

SHREC'13~\cite{li2014comparison} &  \checkmark  & 7200 sketches, 1258 3D models & 90  &   &  o &   & class     &   \\

SHREC'14~\cite{li2014shrec} &  \checkmark  & 12680 sketches, 8987 3D models & 171  &   & o  &   & class &   \\

PACS DG~\cite{Li_2017_ICCV} &  \checkmark  & \tabincell{c}{ 9991 (sketches, photos, \\ cartoons, paintings)}  &  7 &   & o  &   &  class &  domain generalization \\

Flickr1M~\cite{xiao2015sketch} &   & 500 sketches, 1.3M photos  &  100 &   &  o &   & class  &   \\


Cross-Modal Places~\cite{castrejon2016learning} &  \checkmark  & \tabincell{c}{16K sketches, 11K descriptions,\\ 458K spatial texts, 12K clip arts, \\ 1.5M photos}  & 205  &   & s  &   & class &   \\

DomainNet~\cite{peng2019moment} &  \checkmark  & \tabincell{c}{ 0.6M (cliparts, infographs, \\paintings, 	QuickDraw skteches, \\ real photos,\\ professional pencil sketches)}  & 345  & \checkmark  & o &   & class &   \\
\hline

\end{tabular}
}
\end{center}

\end{table*}


==> tex_files/deep_shallow_comparison_table.tex <==
\begin{table}[!t]

\caption{Notation definitions~and abbreviated terms in this survey.}
\label{table:definitions}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ l | l }
\hline
Notations & Descriptions \\
\hline
${\bf M}$, ${\bf M}^{T}$ & matrix ${\bf M}$ and its transpose \\
$\mathcal{X} = \{{\bf X}_{n}\}_{n=1}^{N}$ & sketch sample set \\
${\bf X}_{m}$, ${\bf X}_{n}$ & $m$-th and $n$-th sketch samples in the sketch sample set $\mathcal{X}$ \\
$\mathcal{Y} = \{y_{n}\}_{n=1}^{N}$ & associated label set of $\mathcal{X}$\\
$y_{n}$ & label of ${\bf X}_{n}$ \\
$\mathcal{L}$ & loss function \\
${\bf \Theta}$ & learnable parameters of neural network \\ 
$\mathcal{F}(\cdot)$ & function mapping or feature extraction \\ 
$\mathcal{F}_{\Theta}(\cdot)$ & neural network feature extraction, parameterized by $\Theta$ \\ 
$\mathcal{D}(\cdot, \cdot)$ & distance metric, \eg, $\ell_{2}$ distance \\ 
$\lambda$ & weighting factor \\
$\sum$ &  summation \\
$\alpha$, $\beta$, $\gamma$  & hyper parameters by manually setting \\

\hline
\hline
Abbreviated Terms & Descriptions \\
\hline
CNN &  convolutional neural network \\
GNN & graph neural network \\
RNN & recurrent neural network \\
TCN & temporal convolutional neural network \\
\hline
\end{tabular}
}
\end{center}

\end{table}

==> tex_files/network_architecture.tex <==
\begin{table}[!t]
\scriptsize
\caption{Sketch-oriented network architectures.}
\label{table:architecture_comparison}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ c | c | c }
\hline
Year & Architecture & References \\
\hline
2015  &  CNN  &  \cite{yusketch2015BMVC,yu2017sketch}  \\
2016  &  CNN$\rightarrow$RNN  &  \cite{sarvadevabhatla2016enabling}  \\
2017  &  RNN  &  \cite{xu2018sketchmate} \\
2017 &  CNN feature based RNN-RNN dual branch & \cite{jia2017sequential} \\ 
2017 & RNN (Deep Visual-Sequential Fusion model (DVSF)) & \cite{he2017sketch} \\
2018  &  CNN-RNN dual-branch  &  \cite{xu2018sketchmate}  \\
2018 & binary convolutional neural network &  \cite{prabhu2018distribution}   \\
2018  &  RNN$\rightarrow$CNN  &  \cite{li2018sketch}  \\
2018 &   SketchPointNet & \cite{wang2018sketchpointnet} \\
2019 & multi-graph transformer / GCN & my ArXiv\\
2019 &  photo domain cousin network  via adversarial training, \blue{attribute warehouse}  &     \cite{zhang2019cousin} \\
\hline
\end{tabular}
}
\end{center}

\end{table}

==> tex_files/sketch-generation-frameworks.tex <==
\begin{table*}[!h]
\caption*{{TABLE \todo Comparison of the representative sketch generation deep models.
``gen.'', ``rec.'', and ``com.'' denote ``generation'', ``reconstruction'', and ``completion'', respectively.} \blue{``RNN+VAE'' means ``RNN backbone based VAE''.}}
\label{table:sketch-generation-frameworks}
\begin{center}
\resizebox{\textwidth}{!}{
%\color{blue}
\begin{tabular}{ l || c | c | l}
\hline
\blue{Pipelines} & Representative Ref. & Applications & Advantages \& Disadvantages \\
\hline
\blue{RNN+VAE} & SketchRNN~\todo &  gen., rec., com. & \tabincell{l}{A: brief, flexible. \\    D: scribble effect, single-class gen.} \\
\blue{RNN+GAN} & SkeGAN~\todo & gen., com. & \tabincell{l}{A: less scribble effect, faster convergence. \\   D: single-class gen.}  \\
\blue{RNN+VAE+GAN} & VASkeGAN~\todo &  gen., rec., com. & \tabincell{l}{ A: less scribble effect. \\     D: high complexity, single-class gen., slower convergence}  \\
BERT & \tabincell{l}{Sketchformer~\todo \\ Sketch-BERT~\todo  } &  gen., rec., com.  & \tabincell{l}{A: good at handling longer stroke sequences  \\    D: more parameters, high complexity}  \\
\blue{CNN+RL} & Doodle-SDQ~\todo & imitating a reference  & \tabincell{l}{A: can handle unseen classes.   \\     D: hybrid training (supervised learning \& RL), high complexity}  \\
\hline
\end{tabular}
}
\end{center}

\end{table*}

==> tex_files/task-differences.tex <==
\begin{table*}[!t]
\caption{{ Differences between sketch-based and photo-based single-modal tasks.}}
\label{table:task-differences}
\begin{center}
\resizebox{\textwidth}{!}{
%\color{blue}
\begin{tabular}{ l || c | c || c}
\hline
\multirow{2}{*}{Tasks} & \multicolumn{2}{c||}{Differences}  & \multirow{2}{*}{Reasons}   \\
\cline{2-3}
   &     sketch     &    photo  &   \\
\hline
\hline
%\multirow{3}{*}{Deep Learning} 
recognition &   full-sketch (offline) and partial-sketch (online) recognitions  &    full-photo recognition & partial sketch  could express complete semantics \\
retrieval &   full-sketch (offline) and partial-sketch (online) retrievals & full-photo retrieval    & partial sketch  could express complete semantics   \\
generation &   picture-level and stroke-by-stroke generations &  picture-level generation    &  sketching is a stroke-by-stroke temporal processing \\
segmentation &  pixel-level and stroke-level segmentations &  pixel-level    segmentation &  stroke is the basic semantic unit of sketch \\
\hline
\end{tabular}
}
\end{center}

\end{table*}
